The growing amplification of social media: Measuring temporal and social contagion dynamics for over 150 languages on Twitter for 2009-2020

Working from a dataset of 118 billion messages running from the start of 2009 to the end of 2019, we identify and explore the relative daily use of over 150 languages on Twitter. We find that eight languages comprise 80% of all tweets, with English, Japanese, Spanish, and Portuguese being the most dominant. To quantify social spreading in each language over time, we compute the 'contagion ratio': The balance of retweets to organic messages. We find that for the most common languages on Twitter there is a growing tendency, though not universal, to retweet rather than share new content. By the end of 2019, the contagion ratios for half of the top 30 languages, including English and Spanish, had reached above 1 -- the naive contagion threshold. In 2019, the top 5 languages with the highest average daily ratios were, in order, Thai (7.3), Hindi, Tamil, Urdu, and Catalan, while the bottom 5 were Russian, Swedish, Esperanto, Cebuano, and Finnish (0.26). Further, we show that over time, the contagion ratios for most common languages are growing more strongly than those of rare languages.

==> sections/flipbook.tex <==
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2009.pdf}
\caption{ 
\textbf{Dataset statistics (2009).} Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2009. 
}
\label{fig:stats_2009}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2010.pdf}
\caption{ 
\textbf{Dataset statistics (2010).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2010. 
}
\label{fig:stats_2010}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2011.pdf}
\caption{ 
\textbf{Dataset statistics (2011).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2011. 
}
\label{fig:stats_2011}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2012.pdf}
\caption{ 
\textbf{Dataset statistics (2012).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2012. 
}
\label{fig:stats_2012}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2013.pdf}
\caption{ 
\textbf{Dataset statistics (2013).} Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2013. 
}
\label{fig:stats_2013}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2014.pdf}
\caption{ 
\textbf{Dataset statistics (2014).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2014. 
}
\label{fig:stats_2014}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2015.pdf}
\caption{ 
\textbf{Dataset statistics (2015).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2015. 
}
\label{fig:stats_2015}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2016.pdf}
\caption{ 
\textbf{Dataset statistics (2016).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2016. 
}
\label{fig:stats_2016}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2017.pdf}
\caption{ 
\textbf{Dataset statistics (2017).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2017. 
}
\label{fig:stats_2017}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2018.pdf}
\caption{ 
\textbf{Dataset statistics (2018).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2018. 
}
\label{fig:stats_2018}   
\end{figure*} 
\begin{figure*}[!th]
\includegraphics[width=\textwidth]{figures/stats_2019.pdf}
\caption{ 
\textbf{Dataset statistics (2019).} 
Average number of messages captured daily in our dataset 
as classified by FastText LID algorithm
for 2019. 
}
\label{fig:stats_2019}   
\end{figure*} 

==> sections/flotsam/outtakes_extras.tex <==

Quotations are often used for numerous number of reasons. 
For example, we share quotes with our friends and colleagues to inspire from. 
Academics cite others standing on the shoulders of giants and reshaping our future.
People may quote scientists and politicians to acknowledge their contributions. 
Fans post and re-post information about their favorite movies, and their favorite bands
to share their stories. 
The exercise of 
quoting---repeating someone's else words (e.g., retweeting in the context of 
Twitter)---is in itself a spreading event de novo. 
Different languages, however, will have different cultural norms around this profoundly 
ancient phenomenon that dates back to centuries ago. 
Recent development of social media 
has enabled this contagious behaviour to be observed on a larger scale. 
Many studies address theoretical models of social contagion but without adequate data---in as many different written languages, the dominant mode of online human communication, as is practical---these theoretical modeling studies cannot be effectively confronted with reality.
In this work, we explore and investigate a macroscopic description of social contagion 
through the use of retweets across languages on Twitter. 
We demonstrate how the very practice of retweeting 
varies across different languages.
We study how retweeting naturally lens itself to micro-level discussions of social contagion
on Twitter, which can also be extended to other social media outlets with similar features. 


Social contagion dynamics are studied through the lens of network science, 
statistical mechanics, and computational sociology.
Though we can not give an exhaustive review of this subject here,
we provide background to familiarize the reader and place our work in context.

Although the analogy that ideas can spread and replicate~\cite{ugander2012structural,cozzo2013contact, bessi2015science}
just like viruses is not perfect, it does capture the essence of social contagion.
This observation has widespread application in fields such as 
marketing~\cite{van2007new,trusov2009effects,iyengar2011opinion},
finance~\cite{kelly2000market,cipriani2008herd,hirshleifer2009thought,fenzl2012psychological},
sociology~\cite{hamilton1981models,bovasso1996network,fagan2007social},
and medicine~\cite{christakis2013social,papachristos2015tragic,pollack2017impact}.
Because it can be easier to access data on human social behavior from social media outlets 
than from other sources such as in-person or text-message conversations,
social contagion dynamics are often studied in the context of messages posted 
and subsequently re-posted on social media
platforms~\cite{lerman2010information,romero2011differences,bond201261,kramer2014experimental,ellison2014cultivating,ferrara2016rise}.

The flow of information in the context of social contagion on digital media outlets, 
especially Twitter, has been widely studied in the past few years~\cite{lerman2010information,lerman2012social,hodas2014simple}.
Several models have been proposed to predict the spread of information on Twitter~\cite{zaman2010predicting},
and some other models show the differences in which various topics can propagate throughout social networks~\cite{romero2011differences}. 
Studies have also investigated the extent by which information spread on Twitter 
can have an echo chamber effect~\cite{colleoni2014echo,barbera2015tweeting,barbera2015birds}.


Twitter is a well-structured streaming source of sociotechnical data allowing for the study of dynamical linguistics and cultural phenomena~\cite{zubiaga2015real,dewhurst2020shocklet}.
Of course, like many other social platforms, Twitter represents 
only a subsample of the publicly declared views of utterances, and interactions
of millions of individuals, organizations, 
and automated accounts (Twitter social bots) around the world~\cite{mellon2017twitter,ke2017scientistsonTwitter,mitchell2019reaction,wojcik2019sizing}. 
Researchers have, nevertheless, shown that Twitter's collective 
conversation mirrors the dynamics of local and global events~\cite{palen2016crisis} including
earthquakes~\cite{sakaki2010earthquake},
flu and influenza~\cite{lampos2010tracking,Culotta2010towards}, 
crowdsourcing and disaster relief~\cite{pickard2011time,gao2011harnessing},
major political affairs~\cite{steinert2015online,cody2016public},
and fame dynamics for political figures and celebrities~\cite{dodds2019fame}.
Moreover, analyses of social media data and digital text corpora over the last decade
have advanced natural language processing (NLP) research~\cite{ritter2011named,ritter12open,hirschberg2015advances},
sentiment detection~\cite{dodds2011happiness,chu2012detecting,kryvasheyeu2016rapid},
and word embeddings~\cite{pennington2014glove,devlin2018bert,mikolov2018advances,grave2018learning}.

Twitter has a complex anatomy~\cite{kwak2010twitter}, 
enabling millions of users to communicate freely and spread their information
(e.g., digital social contagion). 
One of the earliest analysis of Twitter by Kwak~et~al.~\cite{kwak2010twitter} suggests that a retweet can reach an average of a thousand users 
regardless of the social network of its original author, spreading its content instantly across different hubs of the full Twitter social network.
Their work shows how retweeting is an effective way to pass on information beyond one's own social network. 


Though research of social contagion sometimes focus on the spreading of specific types of messages, such as 
rumours~\cite{borge2012absence,kwon2013prominent,ozturk2015combating,kaligotla2015agent,zubiaga2016analysing} 
or misinformation (``fake news'')~\cite{del2016spreading,spohr2017fake,shao2017spread,tornberg2018echo},
the fundamental dynamics of idea replication are also interesting.
Users of social media platforms (e.g., Twitter) are faced with a choice:
Post nothing at all; post something original; 
or re-post (``retweet'' in the case of Twitter) an existing post.
The act of retweeting is a spreading event that, 
if replicated in the aggregate, can lead to that idea being a dominant idea on the platform.

Researchers have argued that retweeting is a key mechanism of social contagion on 
Twitter~\cite{nagarajan2010qualitative,stieglitz2012political}.
Suh~et~al.~\cite{suh2010want} examine a set of 74 million tweets to identify contextual features of retweets and retweet rates. 
They show strong association of links and hashtags with retweets. 
Boyd~et~al.~\cite{boyd2010tweet} investigate different styles and drivers of retweeting.
In particular, they argue that the practice of retweeting has become a convention on Twitter 
to spread information, especially for celebrities.
They also show that retweeting is not only an act in which users 
can spread information, but rather a mechanism 
for actors to get involved in a conversation without being an active participant. 


Before we get into investigating the interplay of social contagion across languages, 
we start by exploring the literature around language identification and detection (LID). 
We discuss the state-of-the-art tools that are often used for language detection 
of short and informal messages (e.g., tweets).
We then describe our dataset and our processing pipeline to 
answer some key questions regarding the social contagion through the use of retweets.
Unlike previous studies of language evolution on Twitter~\cite{hong2011language},
in this work, we use FastText~\cite{joulin2016bag,joulin2016fasttext}
to identify and explore the evolution of over 150 languages in over $118$ billion messages collected via
Twitter's 10\% random sample (decahose) from 2009 to 2020~\cite{twitter_api}.
For messages posted after 2013, we also analyze language labels provided by Twitter's proprietary LID algorithm
to justify using FastText as an alternative LID tool 
to overcome the challenge of missing language labels in the historical feed from Twitter. 
We study the empirical dynamics of replication: 
The rate at which users choose to retweet instead of generate original content; 
and how that rate varies across languages temporally.
We quantify the ratio of retweets to new messages (contagion ratio) in each language. 
In most common languages on Twitter, we show that this ratio reveals a growing tendency to retweet.
Finally, we present some analytical results related to the contagion dynamics of Twitter. 





==> sections/gain.tex <==
\subsection{Gain (Ratio Amplifier)} \label{sec:gain}

\begin{figure*}[!th] 
\includegraphics[width=.85\textwidth]{figures/gain_ts.pdf}
\caption{
\textbf{Timeseries for organic messages (blue), retweeted messages (orange), and gain (red) for all languages.}
We show monthly average of all messages on the platform as a function of time.
The blue and orange lines show a monthly average relative rate of usage for organic messages (\textit{tweets}, \textit{replies}, \textit{comments}), and retweeted messages respectively. 
The red line highlights the steady rise of the gain of retweeted messages $G^{(c)}_{\textnormal{messages}}$ as defined in Section~\ref{sec:gain}. 
Inset \textbf{(B)} shows the number of organic messages compared to retweeted messages.
The areas shaded in light grey starting from early 2018 highlights an interesting shift on the platform where the number of retweeted messages exceed the number of organic messages in our dataset. 
An interactive version of the figure for all languages is available in an online 
appendix:
\href{http://compstorylab.org/share/papers/alshaabi2020a/gain\_timeseries.html}{http://compstorylab.org/share/papers/alshaabi2020a/gain\_timeseries.html}
}
\label{fig:gain_ts}    
\end{figure*} 

\begin{figure*}[!th]  
\includegraphics[width=\linewidth]{figures/gains.pdf}
\caption{
\textbf{Annual average of gains as a function of number of messages by language.}
Evidently, we see the same sort of exponential relationship between number of messages and gain of retweeted messages as the one seen in ratio-space.
Unlike ratio, using gain allows us to account for the usage of every language in the dataset with respect to other languages on the platform.
} 
\label{fig:gains}   
\end{figure*} 
   
   
\begin{figure*}[!ht]  
\includegraphics[width=\textwidth]{figures/gain_heatmap.pdf}
\caption{
\textbf{Timelapse of gains.} 
Here we show average gain as a function of time for the top 30 ranked languages of 2019.
Every cell represents average gain of every quarter of the year.
Colored cells indicate a gain higher than 1 whereas gain values below 1 are colored in white.
}
\label{fig:gain_heatmap} 
\end{figure*} 


We define the `contagion ratio’ $R^{(c)}_{\textnormal{\textnormal{messages}}}(\ell)$ as the ratio of retweeted messages to organic messages (Eq.~\ref{eq:contagion_ratio}). 
The contagion ratio 
is an intuitive and interpretable analytical measure.
Alternatively, we can borrow the concept of \textit{gain} from signal processing to take a closer look at this interesting emerging behaviour of language dynamics on the platform.

Let $\mathcal{A}_t$ be the amount of signal observed at time step $t$ for a given arbitrary system,
where $\mathcal{X}_t$ is the contribution of the process we're interested in measuring,
and $\mathcal{O}_t$ represents the amount of remaining signal such that:
\begin{align}
\mathcal{A}_t &= \mathcal{X}_t + \mathcal{O}_t.
\end{align}

Gain is then formally defined as
\begin{align}
G_{\mathcal{X}}^{(t)} &= 10\log_{10} \bigg( \frac{\mathcal{A}_t}{\mathcal{A}_t - \mathcal{O}_t} \bigg).
\end{align}
Hence, gain measures the increase of $\mathcal{X}_t$
with respect to the amount of signal passed through the system.
We note that the leading factor of 10 is simply a constant carried over from conversion to logarithmic Decibel (dB) units. 
In our application, however, we can redefine gain such that:
\begin{align}
    G^{(c)}_{\textnormal{messages}}(\ell) = 10 \log_{10} \left[ \dfrac{\mathcal{C}^{(AT)}_{\ell,t}}{\mathcal{C}^{(OT)}_{\ell,t}} \right],
\end{align}
where $\mathcal{C}_{\ell,t}$ represents the number of messages captured between time step $t - 1$ and time step $t$ for a given target language $\ell$. 

Similar to our observation of the contagion ratio,
gain manifests the same behaviour indicating an increasing marketshare for retweeted messages on the platform, particularly after 2018 (see Fig.~\ref{fig:gain_ts}). 
More importantly, gain represents an analytical approach of investigating the rise of retweeted content among different languages relative to the overall usage, or the number of messages captured for each language.  
Unlike ratio, gain allows us to factor in the number of messages for any given language, and normalize out organic messages to explore how the signal of retweeted messages changes as the number of organic messages up or down.

Again, the trend of retweeted messages is readily seen among most languages on Twitter as shown in both Fig.~\ref{fig:gains} and Fig.~\ref{fig:gain_heatmap}.
This time, however, gain offers a much finer resolution than ratio to explore this dramatic change over time. 
Compiling everything together, 
Fig.~\ref{fig:gains} shows average gain of retweeted messages as a function of the number of messages by language. 
One can arguably view this as a multi-objective optimization task to investigate whether maximizing spread of information (contagion ratio) is correlated with maximizing the number of message for a given language.
We note that a similar sort of scaling between number of messages and gain is evidently seen here as well. 
In fact, using gain we can see that the common languages on the platform with high values of gain now lie on the Pareto-Front (see Fig.~\ref{fig:gains}, 2019). 
Points on the Pareto frontier are not dominated by any other points. 
In other words, \verb|kn| is not on the Pareto frontier because it is dominated by several points, whereas \verb|en|, \verb|es| are not dominated by any other languages in 2019, and thus lie on the Pareto front.
Moreover, the spread of languages in the gain-space seems 
to be growing in time. 
Although the trend for larger slope of gain as a function of number of messages continues to go up over time, 
the variance at the higher end of number of messages also seems to be increasing.

Furthermore, the finer resolution of gain compared to ratio becomes very apparent 
when we look at the heatmap of the average gain 
of retweeted messages in Fig.~\ref{fig:gain_heatmap}.
We show average gain of every quarter of the year
for the top 30 most used languages on Twitter in 2019.
Some languages started to exhibit such behaviour as early as 2010. 
Among many other languages, Thai and Hindi seem to have the most dramatic shift in terms of the number of retweeted messages starting in early 2014. 
A few languages, on the other hand, exhibit major spikes only within specific years.
For example,
Indonesian has a spike that starts late 2010 and continue for about a year.
Similarly, Arabic has a subsequent spike around 2014 followed by a spike in Turkish that starts in 2016 and peaks in late 2017.   


==> sections/model.tex <==

\begin{figure*}[tp!]  
\includegraphics[width=\textwidth]{figures/predictions.pdf}
\caption{
\textbf{Contagion ratio of retweeted messages to organic messages as a function of number of messages by language.}
Although we included all languages in our analysis,
here we only display points corresponding to languages with a ratio value $\in (0, 1)$ to focus on the dynamics of this region of ratio-space.
We fit a multi-stage Bayesian dynamic general linear model to this data.
We describe the model in Appendix \ref{sec:stats}.
There is a significant logarithmic scaling relationship between the number of messages and the contagion ratio.
The expected value of the slope of the linear model increases in each year under study.
We perform out-of-sample predictions and forecast that this increase in slope will continue throughout the year 2020.
}  
\label{fig:predictions}   
\end{figure*} 



\section{Details of the statistical model}
\label{sec:stats}


We fit a multi-stage Bayesian dynamic general linear model (GLM) to model the relationship between $\log_{10} N$ and $R^{(c)}_{\textnormal{\textnormal{messages}}}(\ell)$.
We have denoted number of messages by $N$.
Though $N$ is a discrete quantity, $\log_{10} N$ is a real-valued random variable,
hence our usage of continuous latent variables throughout the model.
We subscript variables with $t$ to denote explicit dependence on time $t$ measured in years.
The model is composed of several pieces. 

We model the generative process of $\log_{10} N$ as 
$\log_{10} N_t \sim \text{Skew-Normal}(\mu_t, \tau_t, \alpha_t)$.
The parameter $\mu_t$ is the mean, while $\tau_t$ is the precision (inverse variance) and $\alpha_t$ is the skew.
We chose a skewed-normal distribution because, though the distribution of $\log_{10} N$ does not have heavy tails, it does exhibit nonzero skew.
Though we use the observed $\log_{10} N$ as the design variable in the GLM component of the model and not the latent $\mu_t$,
we model  $\log_{10} N$ because we want to predict out-of-sample $\log_{10} N$ for $t = 2020$, which we accomplish using the predicted 
$\mu_t$, $\tau_t$, and $\alpha_t$.
We modeled the parameters of the skew-normal distribution using moderately-informative priors which we chose by inspecting the data:
$\mu_t \sim \text{Normal}(5, 1)$, $\tau_t \sim \text{Gamma}(10, 1)$,
and $\alpha_t \sim \text{Normal}(1, 1)$.


Given $\log_{10} N$, we fit a GLM of the form 
$R^{(c)}_{\textnormal{\textnormal{messages}}}(\ell t)
\sim \text{Laplace}(\beta_{0t} + \beta_{1t} \log_{10}N_{\ell,t}, b_t)$.
We chose Laplace-distributed errors to account for the increased variance 
and heteroskedasticity in the distribution of $R^{(c)}_{\textnormal{\textnormal{messages}}}(\ell)$; we are concerned with the median behavior of this distribution for the 
purposes of this model, not the effects of outliers on the model.
We placed centered normal priors on the regression coefficients,
$\beta \sim \text{Normal}(0, 1)$,
and a weakly-informative prior on the scale parameter,
$b \sim \text{Inverse-Gamma}(6, 1)$.
We fit a GLM of this form for each year $t \in \{2009,...,2019\}$.


We believe it is unlikely that the parameters of each GLM are independent of the parameters of the previous GLM; parameters of years $t + 1$ likely depend on parameters of year $t$.
Collecting the vector of parameters as 
$z_t = (\mu_t, \tau_t, \alpha_t, \beta_{0t}, \beta_{1t}, b_t)$,
we model this intertemporal dependence as 
$z_t \sim \text{Multivariate-Normal}(z_{t-1}, L)$. 
The lower triangular matrix $L$ is the Cholesky decomposition of the covariance matrix 
of this process. 
The covariance matrix is given by $\Sigma = \sigma^T R \sigma$,
where 
$\sigma \sim \text{Log-Normal}(0, 1)$ (the isotropic multivariate lognormal distribution)
and the correlation matrix $R \sim \text{LKJ}(\eta)$, with $\eta = 2$.
The density of the LKJ distribution is given as $p(R) \propto |R|^{\eta - 1}$.
We construct pseudo-observations for this process using the expected values of each 
of the parameters at each timestep.
That is, we fit the parameters of the random walk using the pseudo-observations
$$
E[z_t] = \int\ dz_t\ z_t\ p(z_t|\log_{10}N_t, R^{(c)}_{\textnormal{\textnormal{messages}}}(t)),
$$ generated by the posterior.
We did this to reduce the time complexity of model fitting.


After fitting the random walk model, we are able to forecast the statistical relationship between $\log_{10}N_t$ and $R^{(c)}_{\textnormal{\textnormal{messages}}}(t)$ for $t = 2020$.
We evolve the random walk one step (one year) forward in time, and then use the predicted values of $\mu_t$, $\tau_t$, and $\alpha_t$ to generate a synthetic dataset of $\log_{10} N_t$.
We then apply the GLM to this dataset using the predicted values of $\beta_{0t}$, $\beta_{1t}$, and $b_t$.

